Multi-skill Collaborative Teams based on Densest Subgraphs

We consider the problem of identifying a team of skilled individuals for collaboration, in the presence of a social network. Each node in the social network may be an expert in one or more skills. Edge weights specify affinity or collaborative compatibility between respective nodes. Given a project that requires a set of specified number of skilled individuals in each area of expertise, the goal is to identify a team that maximizes the collaborative compatibility. For example, the requirement may be to form a team that has at least three databases experts and at least two theory experts. We explore team formation where the collaborative compatibility objective is measured as the density of the induced subgraph on selected nodes. The problem of maximizing density is NP-hard even when the team requires individuals of only one skill. We present a 3-approximation algorithm that improves upon a naive extension of the previously known algorithm for densest at least $k$ subgraph problem. We further show how the same approximation can be extended to a special case of multiple skills. Our problem generalizes the formulation studied by Lappas et al. [KDD '09] who measure team compatibility in terms of diameter or spanning tree costs. Experiments are performed on a crawl of the DBLP graph where individuals can be skilled in at most four areas - theory, databases, data mining, and artificial intelligence. In addition to our main algorithm, we also present heuristic extensions to trade off between the size of the solution and its induced density. These density-based algorithms outperform the diameter-based objective on several metrics for assessing the collaborative compatibility of teams. The solutions suggested are also intuitively meaningful and scale well with the increase in the number of skilled individuals required.

==> conclusions.tex <==
%\section{Conclusions}
%
%Conclusions - todo atish.
%
%{\bf Acknowledgements.} We would like to thank anonymous reviewers for helpful comments.

==> diameterobjective-oldproof.tex <==
\section{Diameter-based objective}
\label{sec:theory2}
In this section, we mention theoretical results for {\it Diameter-sTF} and {\it Diameter-mTF}. We show that these problems are NP-hard (note that the NP-hardness of {\it Diameter-sTF} does not follow from any previous work). We further present an algorithm {\it MinDiameter} (Algorithm ~\ref{algo:minDia})  which is an extension of {\it RarestFirst} in~\cite{LLT}, and prove that it achieves a 2-approximation factor.
%Note that the NP-hardness of {\it Diameter-sTF} does not follow from any previous work. However, due to space constraints the proofs are omitted in this draft.

\begin{algorithm}[]\label{algo:minDia}
\caption{MinDiameter(G, {\cal T})} 
\label{algo:minDia}
\begin{algorithmic}[1]
\FOR{each $<a, k> \in T$}
\STATE $S(a) = \{ i \mid a \in X_i \}$
\ENDFOR
\STATE $a_{rare} = \arg \min_{<a, k>\ \in T} |S(a)|$
\FOR{each $i \in S(a_{rare})$}
\FOR{each $<a, k>\ \in T$}
\STATE $R_{ia} = d_k(i, S(a), k)$
\ENDFOR
\STATE $R_i \leftarrow \max_a R_{ia}$
\ENDFOR
\STATE $i^* \leftarrow \arg \min R_i$
\STATE ${\cal X'} = \{ i^* \}$
\FOR{each $<a, k>\ \in T$}
\STATE ${\cal X'} = {\cal X'} \cup \{  Path_k(i^*, S(a), k) \}$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{claim} 
{\it Diameter-sTF} and {\it Diameter-mTF} problems are NP-complete.
\end{claim}
\begin{proof}
The problem {\it Diameter-sTF} is in NP. We prove that it is NP-hard by reduction from the 3-satisfiability problem. Consider a 3-SAT instance, say $\phi = C_1 \wedge C_2 ... \wedge C_m$, where each clause, $C_j = x \vee y \vee z$, and $\lbrace x, y, z \rbrace \in U = \lbrace u_1, \neg u_1, u_2, \neg u_2, \cdot \cdot \cdot, u_n, \neg u_n \rbrace$. Let, $C = \lbrace  C_1, C_2, \cdot \cdot \cdot, C_m \rbrace$. We construct an instance of {\it Diameter-sTF} problem corresponding to the 3-SAT instance $\phi$.

For each $u_i, \neg u_i \in U$, create two corresponding nodes in $G$. For each clause $C_j = x \vee y \vee z$, create five nodes in $G$, say $C_{j1}, C_{j2}, Cx_{j}, Cy_{j}, Cz_{j} $.

\noindent{\it Rule $1$:} For each $u_i$ and $\neg u_i$, set $w(u_i, \neg u_i)$ = 3.

\noindent{\it Rule $2$:} For each clause $C_j = x \vee y \vee z$,  set\\ 
$w(C_{jt}, p)=1$, $w(C_{jt}, \neg p)=2$ $\forall t\in\{1, 2\}$ and $p\in\{x, y, z\}$. \\
%$w(C_{j1}, x) =  w(C_{j1}, y) = w(C_{j1}, z) = 1$ \\
%$w(C_{j2}, x) =  w(C_{j2}, y) = w(C_{j2}, z) = 1$ \\
%$w(C_{j1}, \neg x) = w(C_{j1}, \neg y) = w(C_{j1}, \neg z) = 2$. \\
%$w(C_{j2}, \neg x) = w(C_{j2}, \neg y) = w(C_{j2}, \neg z) = 2$. \\
$w(Cp_{j}, p) = w(Cp_{j}, \neg q) = 1$ $\forall p, q\in\{x, y, z\}$ and $q\neq p$.
%$w(Cx_{j}, x) = (Cx_{j}, \neg y) = w(Cx_{j}, \neg z) = 1$ \\
%$w(Cy_{j}, y) = (Cy_{j}, \neg x) = w(Cy_{j}, \neg z) = 1$ \\
%$w(Cz_{j}, z) = (Cz_{j}, \neg x) = w(Cz_{j}, \neg y) = 1$

\noindent{\it Rule $3$:} For each pair of nodes $(x, y)$ in $G$ such that if $w(x,y)$ is not set either by {\it Rule $1$} or {\it Rule $2$} then set $w(x, y) = 2$ except in the following two cases.
\begin{enumerate}
\item$x\in U$ and $y\in U$, and any pair of variables from $\lbrace x, y, \neg x, \neg y \rbrace$ appear together in some clause $C_j \in C$.
\item $x, y$ correspond to $C_{j1}, C_{j2}$ for some clause $C_j \in C$.
\end{enumerate}
For each $u_i, \neg u_i \in U$, associate a skill $a$ to node $u_i, \neg u_i$. And for each $C_j \in C$, associate a skill $a$ to the nodes $C_{j1}, C_{j2}$. Now, set  $k =  \#variables + 2 \#clauses = n + 2m$.

We claim that $\phi$ has a satisfying assignment iff $G$ has a sub-graph $\cal X'$ with $|{\cal X'} \cap S(a)| \ge k$ and $diameter({\cal X'}) \le 2$. 

The {\it Diameter-sTF} returns a sub-graph $\cal X'$ with minimum diameter and has at least $k$ nodes with skill $a$. If $diameter({\cal X'}) \le 2$ then it contains either $u_i$ or $\neg u_i$ but not both because $d(u_i, \neg u_i) = 3$. Since $k = n + 2m$, for each variable $u_i \in U$, $\cal X'$ contains node corresponding to either $u_i$ or $\neg u_i$ (not both) and for each clause $C_j \in C$, $\cal X'$ contains nodes corresponding to $C_{j1}$ and $C_{j2}$. Now, since $diameter({\cal X'}) \le 2$, it implies that $d(C_{j1}, C_{j2}) \le 2$. Further, if $C_j = x \vee y \vee z$,  because of the way $G$ is constructed:\\
$d(C_{j1}, C_{j2})  =  d(C_{j1}, x) + d(x, C_{j2})$  \\
$= d(C_{j1}, y) + d(y, C_{j2}) = d(C_{j1}, z) + d(z, C_{j2})= 2$.

This implies that at least one of the nodes corresponding to $x, y, z$ in $C_j$ is included in the sub-graph $\cal X'$. 

If we set the corresponding variable(s) in the each clause to $1$, each clause has a satisfying assignment. Therefore, $\phi$ has a satisfying assignment.

Now, assume that $\phi$ has a satisfying assignment, then either $u_i$ or $\neg u_i$ appears in the assignment. Further, for each clause $C_j = x \vee y \vee z$, at least one of the variables is set to $1$. Then $G$ contains a subgraph $\cal X'$ corresponding to the variables such that $\cal X'$ contains $u_i$ or $\neg u_i$ and $C_{j1}, C_{j2}$. Thus, if $\phi$ has a satisfying assignment then {Diameter-sTF} returns the subgraph $\cal X'$ with $diameter({\cal X'}) \le 2$ and $|{\cal X'} \cap S(a)| = k$. 
This completes the proof. The NP-completeness of {\it Diameter-mTF} follows from {\it Diameter-sTF}. 
\end{proof}


\begin{claim}
For any graph distance function $d$ that satisfies the triangle inequality, the algorithm {\it MinDiameter} achieves an approximation factor of $2$ for the {\it Diameter-sTF} and\\
{\it Diameter-mTF} problems.
\end{claim}
\begin{proof}
The analysis we present here is similar to the analysis of the {\it RarestFirst} algorithm presented in ~\cite{LLT}. First, consider the solution $\cal X'$ output by the {\it MinDiameter} algorithm, and let $a_{rare} \in T$ be the skill possessed by the least number of individuals in $\cal X$. Also, let $i^*$ be the individual picked from set $S(a_{rare})$ to be included in the solution $\cal X'$. Now, consider two other skills $a_1 \ne a_2 \ne a_{rare}$ and individuals $i, i' \in \cal X$ such that $i \in S(a_1), i \not \in S(a_2)$ and $i' \not \in S(a_1), i' \in S(a_2)$. If $i, i'$ are part of the team reported by the {\it MinDiameter} algorithm, it means that $d(i^*, i) \le d_k(i^*, S(a_1), k_1)$ and $d(i^*, i') \le d_k(i^*, S(a_2), k_2)$. Due to the way the algorithm operates, we can lowerbound the Cc-R cost of the optimal solution, $\cal X^*$,  as follows: 

\begin{equation}\label{DiaBounds}
d(i^*, i) \le \mbox{Cc-R}({\cal X^*}) \mbox{ and }  d(i^*, i') \le \mbox{Cc-R}({\cal X^*})
\end{equation}
Since we have assumed that the distance function $d$ satisfies the triangle inequality, \\
$d (i, i') \le d(i, i^*) + d(i^*, i')$\\
By applying the bounds given in ~\eqref{DiaBounds}, we get the proposed approximation factor. \\
$d (i, i') \le$ Cc-R($\cal X^*) +$ Cc-R(${\cal X^*}) \le 2 \cdot $Cc-R($\cal X^*$).
\end{proof}

%The algorithm {\it MinDiameter} generalizes the algorithm {\it RarestFirst} described in ~\cite{LLT}. 
Algorithm {\it MinDiameter} is as follows. For each individual, say $i_r \in S(a_{rare})$ where $a_{rare}$ is the rarest skill (the skill with the minimum size support set $S$), and for each skill $a_i \in {\cal T}$, the algorithm finds the distance to all the nodes in the support set $S(a_i)$. Then, for each support set $S(a_i)$, it chooses the $k_i$-size subset of $S(a_i)$ such that the maximum shortest path distance between $i_r$ and the nodes in this subset is minimum among all $k_i$-size subsets of $S(a_i)$. We call this distance as $k_i$-th shortest distance between $i_r$ and $S(a_i)$ and denote it as $d_k(i_r, S(a_i), k_i)$. Further, we denote the set of $k_i$ shortest paths between $i_r$ and each of the nodes belonging to the corresponding $k_i$-size subset of $S(a_i)$ as $Path_k(i_r, S(a_i), k_i)$. Thus, for each $i_r \in S(a_{rare})$ the algorithm has identified $k_i$ nodes of skill $a_i$, thereby forming a possible solution team that satisfies the constraints. Finally, the algorithm then picks one of these solutions that has minimum diameter. 
%The algorithm is presented below in detail. 
The time complexity of the algorithm {\it MinDiameter}, assuming that all pairs shortest paths are pre-computed, is $O(n^2)$.



==> introduction_orig.tex <==
\section{Introduction}
We consider the problem of forming teams for collaborative projects in the context of a social network. Each node in the network is an expert in certain skills that may be of interest to the project, and edges between nodes (possibly weighted) reflect the cohesiveness between users. Two users can collaborate better as a team if they have a high-weight edge (strong affinity for interaction) between them. In this setting, the problem is to identify a set of users to form a collaborative team for a project that requires a specified number of people in each of a set of skills.

Specifically, consider the following setting where a social network of computer scientists is presented. Each user is skilled in a subset of areas between theory, databases and data mining. A company wants to hire people for a predetermined project. The goal of the project requires that the team consists of at least three database researchers, at least two theory researchers, and at least one researcher with expertise in data mining. Presented with the social network where edges reflect collaborative interactions, how should the company go about hiring a team for the project?

A special case of this problem was studied in~\cite{LLT}. They consider team formation when the team requires at most one person each in a set of different skills. Our problem formulation generalizes this by allowing the team to require multiple skilled individuals in any skill. Clearly there are projects where multiple people with specific skills may be desired. It turns out that this generalization makes the problem significantly harder and more interesting. For example, the problem is no longer trivial even when the social network contains users that are either skilled or not skilled in just one specific area. Suppose a project requires eight database researchers, and the social network contains people who are either skilled in databases or not, how does one go about choosing the team? We shall mention the complexity as well as algorithmic results for this special case as well shortly.

A critical question in team formation based on a social network is to determine the collaborative quality of a team. The edges specify the collaborative compatibility of two nodes. However, given a subset of say $k$ nodes in the social network (let us even say these $k$ nodes are connected), how do we know how {\em collaborative} this team is? To tackle this, two objectives were suggested in~\cite{LLT}: one based on the diameter of the subgraph induced by these $k$ nodes, and another based on the spanning tree cost of these nodes. Both these objectives are {\em intuitive} and they show that meaningful results are obtained by optimizing based on their cost functions. In this paper, we suggest a density based objective. We define the collaborative affinity of a team of $k$ nodes to be proportional to the density of the induced subgraph. Later on we present the evaluation of the collaborative compatibility of the resulting teams using various metrics.

Using density as a measure of the quality of an induced subgraph of nodes has certain merits over using diameter or minimum spanning tree costs. The main advantage is the {\em stability}. In the case of diameter or minimum spanning tree costs, just adding one edge between two nodes can radically change the quality of the solution. Similarly, deleting an edge can suddenly reduce the quality of a solution. However, the density of a subset of nodes is smoother in this regard. Adding or deleting an edge only affects the quality of the solution to the extent of the weight of the edge (compared to the {\em total} weight of all the other edges). Also, notice that for density, adding  or deleting an edge necessarily increases or decreases the quality respectively, of the solution. This seems intuitive as an added collaboration between two people in the team enhances the quality of the team. However, in the case of diameter or spanning tree costs, adding or deleting an edge may not affect the solution at all. 
%A possible drawback, however, of density objective compared to the other two is that even a disconnected team (in terms of the induced subgraph) may have a high quality as a solution; it is not clear if this is necessarily a disadvantage.

Briefly, given a set of skills $1, 2, \ldots, t$, and requirements $k_1, k_2, \ldots, k_t$, and a social network of nodes connected by (weighted) edges, the goal is to pick a subset of nodes such that at least $k_i$ distinct nodes possess skill $i$, for $1\leq i\leq t$. The same node, however, may contribute to two different skills. The objective value of the solution is the density of the induced subgraph on these nodes.
%; the edge weights specified as a part of the input. 
The goal is to maximize this objective. Notice that the number of returned nodes may be as small as $k_{max} = \max_{i}{k_i}$ or be even larger than $\sum_{i}{k_i}$. We now summarize the contributions of this paper.

\noindent{\bf Our Contributions.}

\begin{itemize}
\item We present a novel problem definition for team formation to maximize collaborative compatibility. The constraint of the problem requires the team to comprise of at least a {\em specified number} of skilled individuals in each of a set of skills. This generalizes previous work that required forming a team with at least {\em one} skilled individual in each of a set of skills. Further, as a measure of collaborative compatibility, we suggest a density based objective. Density is a novel metric for this domain and we show that it has certain desirable properties for measuring compatibility. Our density based team formation problem also generalizes previous graph algorithms work on finding densest subgraphs with size constraints.
\item We address the collaborative team formation problem when the team requires one or more skills. We show that optimizing even the special case of a single skill is  NP-hard under our density-based metric, as well as the previously suggested diameter-based metric. The main theoretical result of the paper is to present a novel 3-approximation algorithm for the density based team formation problem for both single as well as a special case of multiple skills. This improves upon a naive extension of previous work on size constrained densest subgraph problems. We also show how previous work on a 2-approximation for the diameter-based objective can be extended to our generalized problem.
\item We present several heuristic algorithms that build on our 3-approximation for density-based team formation. These algorithms trade-off between the size of the returned solution and the density, while respecting the constraints on the skill requirements. We perform experiments on all these algorithms on the DBLP graph. Experiments show that density-based algorithms perform well in practice, identifying tightly knit and highly skilled teams and also scale well with the size of the team and skill requirements. We show that the density-based algorithms compare favorably to the diameter-based algorithms on a number of different metrics. We also show through qualitative analysis that the teams suggested are intuitive and meaningful.
\end{itemize}

\noindent{\bf Overview.} We mention related work in Section~\ref{sec:rel}. The various problem definitions, notations and some properties are formalized in Section~\ref{sec:def}. Our theoretical contributions, including the main 3-approximation algorithm for our density based objective are described in Section~\ref{sec:theory1}. The theoretical work on a diameter based objective is presented in Section~\ref{sec:theory2}. Finally, some additional heuristic algorithms and experimental results are detailed in Section~\ref{sec:exp}. 
%Finally, we make some concluding remarks in Section~\ref{sec:con}.

==> problemdef_orig.tex <==
\section{Problem Definition}
\label{sec:def}

%\subsection{Notation} 
\noindent{\bf Notation.}
Let ${\cal X} = \{ 1, \ldots,n \}$ denote a set of $n$ individuals and ${\cal A} =$ \{$a_1, \ldots, a_m$\} denote a set of $m$ skills. Each individual $i$ is associated with a set of skills $X_i \subseteq {\cal A}$. If $a_j \in X_i$, then an individual $i$ has skill $a_j$. For each skill $a$, we define its support set, $S(a)$, as the set of individuals in $\cal X$ with skill $a$. That is, $S (a) = \{ i |  i \in {\cal X}$ and $a \in X_i \}$. A task $\cal T$ is a set of pairs where each pair, <$a_j$,$k_j$>, specifies that at least $k_j$ individuals of skill $a_j$ are required to perform the task.  

Let $G({\cal X}, E)$ denote the undirected, weighted graph representing the social network associated with the set of individuals ${\cal X}$. 
%The weight associated with each edge signifies the collaborative compatibility between the nodes they connect. 
We use the notations $E(G)$ and $V(G)$ to represent the edge set and vertex set associated with the graph $G$. If ${\cal X'} \subseteq V(G)$, we use $G[\cal X']$ to denote the subgraph of $G$ induced by the nodes in $\cal X'$. Further, $W(\cal X')$ denotes the sum of the edge-weights associated with all the edges in the subgraph induced by the nodes in $\cal X'$. We also define a distance function between any two node $i, i'$ in a graph $G$ as the sum of the edge-weights along the shortest path between $i$ and $i'$ in $G$. Further, without loss of generality, we assume that the graph $G$ is connected; we can transform every disconnected subgraph to a connected one by simply adding an edge that denotes zero collaborative compatibility. Given a measure of collaborative compatibility $Cc()$, we now formalize the problems considered in this paper.

%Problem $1$ [{\it Single Skill Team Formation (sTF)}]  \\
\noindent{\bf Single Skill Team Formation (sTF).} Given a set of $n$ individuals ${\cal X} = \{ 1, \ldots, n \}$, a graph $G({\cal X}, E)$, task ${\cal T} =$ \{<a, k>\}, find $\cal X' \subseteq X$, such that $|{\cal X}'  \cap S(a)| \ge k$, and the collaborative compatibility $Cc(\cal X')$ is optimized. 

%Problem $2$ [{\it Multiple Skill Team Formation (mTF)}]  \\
\noindent{\bf Multiple Skill Team Formation (mTF).} Given a set of $n$ individuals ${\cal X} = \{ 1,\ldots, n \}$, a graph $G({\cal X}, E)$, task ${\cal T} =$ \{$<a_1, k_1>, <a_2, k_2>, \ldots, <a_m, k_m>$\}, find $ \cal X' \subseteq X$, such that $|{\cal X}'  \cap S(a_j)| \ge k_j$  for each $j \in \{ 1, \ldots, m \}$ and the collaborative compatibility $Cc(\cal X')$ is optimized.

%We define the following two metrics for collaborative compatibility mentioned in the problems {\it sTF} and {\it mTF}.\\ 

The main metric that we consider for collaborative compatibility for {\it sTF} and {\it mTF} is the following density based objective. In addition to this, we consider a diameter based objective as well (suggested in~\cite{LLT}) for comparison.

\noindent{\bf Maximum Density(D).} Given a graph $G({\cal X}, E)$ and a set of individuals $\cal X' \subseteq X$, we define the density collaborative compatibility of $\cal X'$, denoted by {\it Cc-D}$(\cal X')$ to be the density of the induced  subgraph $G[\cal X']$. Recall that the density $d(G)$ of a graph $G$ is defined as $d(G) = \frac{W(G)}{|V(G)|}$ . The higher the value of the density, the better is the collaborative compatibility. An optimal solution $\cal X' \subseteq X$, is the team that can perform task $\cal T$ and has maximum density. 

\noindent{\bf Minimum Diameter(R).} Given a graph $G({\cal X}, E)$ and a set of individuals $\cal X' \subseteq X$, we define the diameter collaborative compatibility of $\cal X'$, denoted by {\it Cc-R}$(\cal X')$, to be the diameter of the subgraph $G[\cal X']$. Recall that the diameter of a graph is the largest shortest path between any two nodes in the graph. 
%The lower the value of the diameter, the better is the collaborative compatibility. 
An optimal solution $\cal X' \subseteq X$, is the team that can perform task $\cal T$ and has minimum diameter. 

In the following sections, we refer to the {\it Single Skill Team Formation (sTF)} and {\it Multiple Skill Team Formation (mTF)} problems with collaborative compatibility {\it Cc-R} as {\it Diameter-sTF} and {\it Diameter-mTF}, respectively.  Similarly, for the collaborative compatibility {\it Cc-D} we refer to the corresponding problems as {\it Density-sTF} and {\it Density-mTF} respectively.

%\subsection{Properties}
\noindent{\bf Properties.} We now describe some properties of the maximum density objective. 
%These properties are not satisfied by the minimum diameter objective.
For brevity, we mention the intuition without a rigorous definition or proof.

\noindent{\bf Strict Monotonicity.} If a communication edge (with positive weight) is added between two nodes in the solution set for the {\it Density-sTF} or {\it Density-mTF} problem, then the collaborative compatibility objective {\it Cc-D} for the solution necessarily increases. Similarly, if a communication edge already present is deleted, then the {\it Cc-D} objective value decreases. 

\noindent{\bf Sensitivity.} The {\it Cc-D} value for {\it Density-sTF} or {\it Density-mTF} does not increase or decrease radically upon adding or deleting an edge. Specifically, it can only change to an extent depending on the weight of the added or deleted edge, compared to the total weight of edges in the solution. 

Notice that neither of these properties hold on {\it Diameter-sTF} or {\it Diameter-mTF} (or a minimum spanning tree based objective suggested in~\cite{LLT}). For example, adding or deleting an edge may not alter the diameter of the solution and therefore {\it Cc-R} is not monotonic. Similarly, adding or deleting an edge can radically change the diameter (for example make it finite from infinite) for an induced subgraph; this implies that the diameter objective is highly sensitive to small change. 

The properties for density based objectives fall out of the fact that adding or deleting edges only gradually alters the density of a solution subgraph. Diameter based objectives (or even the minimum spanning tree based objective suggested in~\cite{LLT} that we do not consider in this paper) are not smooth in this sense; altering the graph slightly can change the objective radically. These properties make density based objectives somewhat more suitable. One drawback, however, of density as an objective arises from the fact that the optimal solution may contain disconnected components. Notice that this is not the case for the diameter based objective. In the experimental section we suggest the heuristic algorithms to ensure returning connected dense solutions. 

Eventually, the quality of teams produced by different definitions
% (as a set of skilled nodes as well as a potential for collaborative compatibility) 
needs to be evaluated (potential for collaboration) based on the measures neutral to these definitions; we make such objective comparisons in the experimental section.
